DeVIS: Making Deformable Transformers Work for Video Instance Segmentation

Video Instance Segmentation (VIS) jointly tackles multi-object detection, tracking, and segmentation in video sequences. In the past, VIS methods mirrored the fragmentation of these subtasks in their architectural design, hence missing out on a joint solution. Transformers recently allowed to cast the entire VIS task as a single set-prediction problem. Nevertheless, the quadratic complexity of existing Transformer-based methods requires long training times, high memory requirements, and processing of low-single-scale feature maps. Deformable attention provides a more efficient alternative but its application to the temporal domain or the segmentation task have not yet been explored. In this work, we present Deformable VIS (DeVIS), a VIS method which capitalizes on the efficiency and performance of deformable Transformers. To reason about all VIS subtasks jointly over multiple frames, we present temporal multi-scale deformable attention with instance-aware object queries. We further introduce a new image and video instance mask head with multi-scale features, and perform near-online video processing with multi-cue clip tracking. DeVIS reduces memory as well as training time requirements, and achieves state-of-the-art results on the YouTube-VIS 2021, as well as the challenging OVIS dataset. Code is available at https://github.com/acaelles97/DeVIS.

==> figures/backbone.tex <==
\begin{figure}[H]
    \centering\small
    \includegraphics[scale=1.5]{img/images_methodology/def_vistr_backbone.png}
    \caption[\detr Multi-Scale features for Deformable VisTr]{Constructing multi-scale features from the input clip for Deformable VisTr}
    \label{fig:defvistr_backbone}
\end{figure}

==> tables/ablation_clip_size.tex <==
\begin{table*}
\centering

\caption{Different clip sizes $\tau$. YouTube-VIS 2019~\cite{Yang2019vis}}

\label{tab:ablation_clip_size}

\begin{tabular}{c | cccccc}

\toprule

% &&\multicolumn{3}{c|}{$\tau = 3$} & \multicolumn{3}{c|}{$\tau=6$} & \multicolumn{3}{c}{$\tau=9$}\\


    & \multicolumn{5}{c}{AP} \\
% \cmidrule{2-6}
\midrule
% $\tau$    &$\tau = 3$ & $\tau = 6$ & $\tau = 9$ & $\tau = 18$ & $\tau = 36$ \\
$\tau$    & 3 & 6 & 9 & 18 & 36 \\



\midrule
% $K_{temp}=0$ & X & X & X & X & X\\
$K_{temp}=4$ & X & X & X & X & X\\
%&$K_{t}=4$ &X &X &X &X &X &X &X &X &X \\
\bottomrule
\end{tabular}


\end{table*}

==> tables/ablation_encoder_archs.tex <==
% Table 4) Value we bring to the encoder. On this table i propose to use each of the transformers encoder presented by each of the other architectures. This should really make clear how powerful the temporal connections are: we should of course have more performance than no connections (same encoder as SeqFormer) but it is interesting to see the comparison with inter frame communications transformers. 
\begin{table*}

    \caption{Different encoder configurations.  $W$ stand for the temporal window used and $K_{t}$ the number of temporal points. We use clip size $T=6$}
    
    \center
    % \setlength{\tabcolsep}{14.0 pt}
    \begin{tabular}{@{}ccc|cccc@{}}\toprule
    &&&AP &AP$_{75}$ &AP$_{50}$\\
    \midrule
    \multicolumn{3}{c|}{Full THW}&X &X &X\\
    midrule
    \multicolumn{3}{c|}{IFC}&X &X &X\\
    \midrule
    \multicolumn{3}{c|}{Spatial MS Def Att.}&X &X &X\\
    \midrule
    \multirow{4}*{Temp. MS Def. Att.}
    \multirow{2}*{$W=2$} &&$K_{t}=2$ &X &43.2 &X\\
    &&$K_{t}=4$ &X &X &X\\
    \multirow{2}*{$W=4$} &&$K_{t}=2$ &X &X &X\\
    &&$K_{t}=4$ &X &X &X\\
    \bottomrule
    \end{tabular}

\end{table*}

==> tables/ablation_loss_balance.tex <==
\begin{table*}

 \caption{Balanced auxiliary loss strategy and gradient propagation. We prove that balanced loss strategy needs to go together with gradient propagation to see the most benefit from it.}
 \label{tab:ablation_loss_balance}
 
  \center
  \begin{tabular}{cc|ccc}
  \toprule
    Gradient prop. &Balanced loss &AP &AP$_{75}$ &AP$_{50}$\\
  \midrule
  \xmark &\xmark &$X$ &$X$  &$X$ \\
  \xmark &\checkmark &$X$ &$X$  &$X$ \\
  \checkmark &\checkmark &$X$ &$X$  &$X$ \\
  \bottomrule
 \end{tabular}
\end{table*}

==> tables/ablation_main_old.tex <==
\begin{table*}[t]

\caption{
Ablation of our main ~\textbf{\evis{} contributions} and the incremental built from a naive Deformable~\vistr{} to our final model.
%
\textit{Increase spatial inputs} denotes a training on higher input resolutions.
% All experiments use encoder $K_2=2$ and decoder $K_2=1$.
%
% We use the exact same data transformation as VisTr.
%
}

\label{tab:ablation_main}

\centering

\resizebox{\columnwidth}{!}{%

\begin{tabular}{lrccc | cccHc}

\toprule

%&\thead{Loss \\ weighting} &\thead{New matcher \\ loss}
% 
%&\thead{Multi-scale \\ mask head}
%&\thead{Spatial \\ adjustments}

Method  &  \thead{Clip \\ size $\tau$}   & $K_{curr}$ & $K_{temp}$  &\thead{Feature \\ scales} & AP & $\Delta$ AP &\thead{Training \\ GPU hours} & FPS &\thead{\#params}\\

\toprule

\vistr  & 36  & All  & All   & 1 & 36.1 & -- & 350 & 69.9 &57M\\

\midrule
\multirow{5}*{\shortstack[l]{Deformable \\ \vistr{}}}       
                    
                    &36  &4  &4    &1   &29.4(32.3)  & -- &260 &64.3 &47M\\
                    
                    % &36  &4  &4    &4  & --     & --   & -- & -- &68M\\
                    
                    &36  & 4  & 0  &1   &31.9(33.8)   & -- &155 &83.2 &36M\\
                    
                    &36  & 4  & 0  &4   &--   & -- &XX &XX &XX\\
                    
                    % &36  & 4  & 0  &4   & XX   & -- &XX &XX &XX\\
                    
%  &36  &6  &6               &360 Object  &     &X  &7hx4  & X &42M\\

                    % &12  &12  &12               & 120 Object &     &X  &X  & X &X\\

                    % &9  &9  &9               & 90 Object  &     &X  &X  & X &X\\

                    &6  &4  &4   & 1 &   34.0   & -- &48  &31.8  &41M\\
                    
                    &6  &4  &0   & 1 &  32.3    & -- &30  &XX  &36M\\

                    % &3  &3  &3               & 30 Object   &    &X  &X  & X &X\\

%\evis{}                    &36  &2  &36             &360 Object&31.4  & &116 & X &X\\

%\evis{}                    & 36  & 2  &36                &360 Object&33.3  &  &116 & X &X\\

%\evis{}                    & 36  &6  &6                    &360 Object&34.3  & &140 & X &X\\

\midrule
\evis{}                             &  &  &     & &   &  && &\\
% \evis{}                             &6  &6  &6     &60 Object &33.9   &63  &13.3 &X\\
+ Increase spatial inputs          &6  &4  &4      & 4 & 35.1  & +1.1  & 93    & 25.5  & 48M\\
+ Instance-aware object queries     &6  &4  &4      & 4 & 36.6  & +1.5  & 112    & 22.3  & 48M\\
+ Multi-scale mask head             &6  &4  &4      & 4 & 40.3  & +3.7  & 120      & 23.4  & 48M\\
+ Multi-cue clip tracking           &6  &4  &4      & 4 & 41.3  & +1.0  & 120      & 18.4  & 48M\\
% + Auxiliary loss weighting, loss all frames  &6  &4  &4  & 4 &44.2  & +2.9  & 3:15hx4   & X  & 48M\\
+ Auxiliary loss weighting  &6  &4  &4  & 4 &44.2  & +2.9  & 120   & 18.4  & 48M\\

\bottomrule

\end{tabular}
}

\vspace{-0.5cm}

\end{table*}

==> tables/ablation_mask_head.tex <==
\begin{table*}[t]
\caption{%
    Ablation for the \textbf{multi-scale mask head} on COCO~\cite{COCO} val 2017.
    %
    Our baseline uses the original mask head architecture as in~\detr{}~\cite{DETR} but applied on top of Deformable~\detr{}~\cite{deformable_detr}.
    %
    % We then show how each newly added component helps improving the performance.
}
\label{tab:ablation_mask_head}
\centering
\input{tables/ablation_mask_head_tabular}

\end{table*}

% Mask RCNN APl APm APs
%53.3, 39.4, 18.6
% APl APm APs
%53.1 36.8 13.5





==> tables/ablation_matcher_loss.tex <==
\begin{table*}
 \caption{Different matching and loss strategies based on how to proceed when an instance is not present in any particular frame.}
 \label{tab:ablation_matcher_loss}
  \center
%   \setlength{\tabcolsep}{5.0 pt}
  \begin{tabular}{ccc|ccc}
  \toprule
     Matcher cost &Bbox/Mask loss &Class. loss &AP &AP$_{75}$ &AP$_{50}$\\
  \midrule
   All frames   &Valid frames &Valid frames &$X$ &$X$  &$X$ \\
   Valid frames &Valid frames &Valid frames &$X$ &$X$  &$X$ \\
   All frames   &All frames   &All frames   &$X$ &$X$  &$X$ \\
   All frames   &All frames   &Valid frames &$X$ &$X$  &$X$ \\
  \bottomrule
 \end{tabular}
\end{table*}

==> tables/ablation_multi_cues.tex <==
% \begin{table*}
%  \caption{Impact of each component from our multi-cue clip tracking/stitching strategy.}
%  \label{tab:ablation_multi_cues}
%   \center
% %   \setlength{\tabcolsep}{5.0 pt}
%   \begin{tabular}{cccH|ccc}
%   \toprule
%     \thead{Volumetric \\ soft IoU} & Class & \thead{Class \\ Score} & \thead{Bounding box \\ center} &$AP$ &AP$_{75}$ &AP$_{50}$\\
%   \midrule
%   \checkmark &\xmark &\xmark &\xmark &$41.6$ &$45.9$  &$61.7$ \\
%   \checkmark &\checkmark &\xmark &\xmark &$41.5$ &$45.6$  &$63.6$ \\
%   \checkmark &\checkmark &\checkmark &\xmark &$43.4$ &$47.8$  &$66.4$ \\
% %   \checkmark &\checkmark &\checkmark &\checkmark &$43.1$ &$47.9$  &$64.6$ \\
% %  \xmark &\checkmark &\checkmark &\checkmark &$41.3$ &$44.7$  &$63$ \\
%   \toprule
%  \end{tabular}
% \end{table*}




\begin{table*}
 \caption{Impact of each component from our multi-cue clip tracking/stitching strategy. \todo{rerun on new best 44.1 config.} YouTube-VIS 2019~\cite{Yang2019vis}}
 \label{tab:ablation_multi_cues}
  \center
  \input{tables/ablation_multi_cues_tabular}
\end{table*}

==> tables/ablation_temporal.tex <==
\begin{table*}[t]

 \caption{
%
Removing \textbf{temporal connections} with $K_{temp}=0$ results in performance drops across all datasets.
%
We observe an optimal clip size of $\tau=6$.
%
%  We evaluate the impact of the temporal connections on the multi-scale deformable attention on each dataset.
%
%  The benefit obtained increases as the dataset difficulty also increases
%
%  \todo{rerun clip size 3 9 12 in final config}.
}
 
 \label{tab:ablation_temporal}
 
  \center
%   \setlength{\tabcolsep}{8.0 pt}
  \input{tables/ablation_temporal_tabular}
 
\end{table*}

==> tables/ablation_topK.tex <==
\begin{table*}
\caption{
    Impact of increasing the value of TopK during inference on YouTube-2019~\cite{Yang2019vis}
}
\begin{center}
\input{tables/ablation_topk_tabular}
\end{center}

\label{tab:ablation_topK}

\end{table*}


==> tables/ablation_topk_tabular.tex <==
\begin{tabular}{l|ccc}
  %\toprule
    TopK  & AP &AP$_{50}$ &AP$_{75}$\\
  \midrule
  10 &$44.0$ &$66.7$ &$48.6$  \\
  20 &$44.4$ &$67.9$ &$48.6$   \\
  30 &$44.4$ &$67.7$  &$49.1$   \\
  40 &$44.3$ &$67.6$  &$48.7$  \\
 \end{tabular}

==> tables/eval_COCO.tex <==
\begin{table*}

\caption{Instance Segmentation results evaluated on COCO~\cite{COCO} val 2017. \mbox{Mask R-CNN} results are extracted from detectron2~\cite{wu2019detectron2} with the 3x schedule configuration. All methods use a ResNet-50~\cite{resnet} backbone.}
\label{tab:eval_COCO}

\center
% \setlength{\tabcolsep}{2.0 pt}
\input{tables/eval_COCO_tabular}
\end{table*}

==> tables/eval_OVIS.tex <==
\begin{table*}

\caption{
A comparison on the challenging \textbf{OVIS}~\cite{ovis} validation set.
%
Our~\evis{} method is superior to all previous approaches by a large margin.
%
% Methods denoted with * apply the temporal calibration module proposed in~\cite{ovis}. 
%
% \todo{rerun best with object queries}
}
\label{tab:eval_OVIS}

\begin{center}
\input{tables/eval_OVIS_tabular}
\end{center}
\end{table*}

==> tables/eval_OVIS_and_COCO.tex <==
\begin{table*}[t]
\parbox[t][][t]{.48\linewidth}{

\centering

\caption{
Comparison on the challenging \textbf{OVIS}~\cite{ovis} validation set.
% Our~\evis{} method is superior to all previous approaches by a large margin.
%
% Methods denoted with * apply the temporal calibration module proposed in~\cite{ovis}. 
%
% \todo{rerun best with object queries}
}
\label{tab:eval_OVIS}

\resizebox{0.48\columnwidth}{!}{%
\input{tables/eval_OVIS_tabular}
}
}\hfill
\parbox[t][][t]{.48\linewidth}{
\centering

\caption{
Comparison of instance segmentation results on the \textbf{COCO}~\cite{COCO} validation set.
%
\mbox{Mask R-CNN} results are from detectron2~\cite{wu2019detectron2}.
%
% \todo{spend a lot of time making these tables look a like only for better alignment. we need text long enough enough enough enough enough enough}
}
\label{tab:eval_COCO}
\vspace{0.17cm}

\resizebox{0.48\columnwidth}{!}{%

\input{tables/eval_COCO_tabular}
}
}
\end{table*}

==> tables/eval_OVIS_tabular.tex <==
\begin{tabular}{l | ccc}
\toprule
Methods & AP & AP$_{50}$ & AP$_{75}$\\
\midrule
STEm-Seg~\cite{stem_seg}  & $13.8$ & $32.1$ & $11.9$ \\
SipMask-VIS~\cite{sip_mask}  & $14.3$ & $29.9$ & $12.5$ \\
MaskTrack R-CNN~\cite{Yang2019vis} & $15.4$ & $33.9$ & $13.1$ \\
CrossVIS~\cite{cross_vis} &$18.1$ & $35.5$ & $16.9$ \\

\midrule 

\textbf{\evis{}} &23.2 &44.0 &21.7\\
\bottomrule
\end{tabular}

==> tables/eval_YTVis-2019.tex <==

\begin{table*}

\caption{
Quantitative evaluation on \textbf{YouTube-VIS 2019}~\cite{Yang2019vis} validation set. etc....
%
\todo{Explain cross for STMask and star for SG-Net}
}

\label{tab:eval_YTVis-2019}

\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l l|l|r|ccccc}
\toprule
\multicolumn{2}{c|}{Methods} & Backbone & FPS & AP & AP$_{50}$ & AP$_{75}$ & AR$_1$ & AR$_{10}$\\

\midrule
\multirow{7}*{Online} & MaskTrack-RCNN & ResNet-50 & 26.1 & 30.3 & 51.1 & 32.6 & 31.0 & 35.5\\
& SipMask & ResNet-50 & 35.5 & 33.7 & 54.1 & 35.8 & 35.4 & 40.1\\
& SG-Net & ResNet-50 & $^{\ast}$23.0 & 34.8 & 56.1 & 36.8 & 35.8 & 40.8\\
& CompFeat & ResNet-50 & $-$ & 35.3 & 56.0 & 38.6 & 33.1 & 40.3\\
& CrossVIS & ResNet-50 & 25.6 & 36.3 & 56.8 & 38.9 & 35.6 & 40.7\\
& STMask & ResNet-50$^{\dagger}$ & 26.1 & 33.5 & 52.1 & 36.9 & 31.1 & 39.2\\
& VISOLO & ResNet-50 & 40.0 & 38.6 & 56.3 & 43.7 & 35.7 & 42.5\\

\midrule
\multirow{4}*{Offline}
& VisTR & ResNet-50 & 51.1 & 36.2 & 59.8 & 36.9 & 37.2 & 42.4\\
& SeqMask-RCNN & ResNet-50 & 3.8 & 40.4 & 63.0 & 43.8 & 41.1 & 49.7\\
& IFC & ResNet-50 & 107.1 & 41.2 & 65.1 & 44.6 & 42.3 & 49.6\\
& SeqFormer & ResNet-50 & \textbf{12} & 45.1 & 66.9 & 50.5 & 45.6 & 54.6\\

\midrule
\multirow{5}*{Near online}
& MaskProp (T=12) & ResNet-50 & - & 40.0 & - & 42.9 & - & -\\
& STEm-Seg & ResNet-50 & 3.0 & 34.6 & 55.8 & 37.9 & 34.4 & 41.6\\
& IFC (T=5, S=1) & ResNet-50 & 46.5 & 39.0 &60.4 &42.7 & 41.7 & 51.6\\
& \textbf{\evis{}} (T=6, S=4) & ResNet-50 & 7.0 & \textbf{43.3} & \textbf{67.9} & \textbf{46.4} & \textbf{42.9} & \textbf{52.3}\\
& \textbf{\evis{}} (T=6, S=4) & ResNet-101 & XX & XX & XX & XX & XX & XX \\

\bottomrule
\end{tabular}}
\end{center}


\end{table*}



==> tables/eval_YTVis-2021.tex <==
\begin{table*}

\caption{
Quantitative evaluation on \textbf{YouTube-VIS 2021} validation set. We refer the results reported in [cite VISOLO]. All models use the ResNet-50~\cite{resnet} as the backbone network, except for STMask~\cite{stmask} that uses ResNet-50-DCN.
}

\label{tab:eval_YTVis-2021}

\begin{center}
\begin{tabular}{l | ccccc}
\toprule
Methods & AP & AP$_{50}$ & AP$_{75}$ & AR$_1$ & AR$_{10}$\\
\midrule
MaskTrack-RCNN &  28.6 & 48.9 & 29.6 & 26.5 & 33.8\\
SipMask & 31.7 & 52.5 & 34.0 & 30.8 & 37.8\\
CrossVIS & 34.2 & 54.4 & 37.9 & 30.4 & 38.2\\
STMask & 30.6 & 49.4 & 32.0 & 26.4 & 36.0\\
IFC & 35.2 & 57.2 & 37.5 &-- &--\\
VISOLO & 36.9 & 54.7 & 40.2 & 30.6 & 40.9\\
% SeqFormer & 40.5 & 62.4 &43.7 &36.1 & 48.1\\

\midrule

\textbf{\evis{}} &41.5 &X &X &X &X\\

\bottomrule
\end{tabular}
\end{center}

\end{table*}
